FedSAF: A Federated Learning Framework for Enhanced Gastric Cancer Detection and Privacy Preservation

Gastric cancer is one of the most commonly diagnosed cancers and has a high mortality rate. Due to limited medical resources, developing machine learning models for gastric cancer recognition provides an efficient solution for medical institutions. However, such models typically require large sample sizes for training and testing, which can challenge patient privacy. Federated learning offers an effective alternative by enabling model training across multiple institutions without sharing sensitive patient data. This paper addresses the limited sample size of publicly available gastric cancer data with a modified data processing method. This paper introduces FedSAF, a novel federated learning algorithm designed to improve the performance of existing methods, particularly in non-independent and identically distributed (non-IID) data scenarios. FedSAF incorporates attention-based message passing and the Fisher Information Matrix to enhance model accuracy, while a model splitting function reduces computation and transmission costs. Hyperparameter tuning and ablation studies demonstrate the effectiveness of this new algorithm, showing improvements in test accuracy on gastric cancer datasets, with FedSAF outperforming existing federated learning methods like FedAMP, FedAvg, and FedProx. The framework's robustness and generalization ability were further validated across additional datasets (SEED, BOT, FashionMNIST, and CIFAR-10), achieving high performance in diverse environments.

==> oldbib <==
@article{niu2024flrce,
  title = {FLrce: Resource-Efficient Federated Learning with Early-Stopping Strategy},
  author = {Niu, Ziru and Dong, Hai and Qin, A. K. and Gu, Tao},
  journal = {IEEE Transactions on Mobile Computing},
  year = {2024},
  doi = {10.1109/TMC.2024.3447000}
}

@article{Wang2023hahnet,
  author = {Wang, Yiqing and Zhang, Lei and Xu, Xiaofei and Chen, Mingyue and Zhang, Jing},
  title = {HAHNet: Multi-scale and Attention-based Network for HER2 Status Classification},
  journal = {Nature Communications},
  volume = {14},
  number = {10},
  pages = {230-240},
  year = {2023},
  doi = {10.1038/s41586-023-00210-8}
}

@article{zitnik2017predicting,
  title = {Predicting multicellular function through multi-layer tissue networks},
  author = {Zitnik, Marinka and Leskovec, Jure},
  journal = {Bioinformatics},
  volume = {33},
  number = {14},
  pages = {i190--i198},
  year = {2017},
  doi = {10.1093/bioinformatics/btx252}
}


@article{hudis2007trastuzumab,
  author = {Hudis, Clifford A.},
  title = {Trastuzumab—mechanism of action and use in clinical practice},
  journal = {New England Journal of Medicine},
  volume = {357},
  number = {1},
  pages = {39--51},
  year = {2007},
  publisher = {Massachusetts Medical Society}
}




@book{american2010publication,
  title={Publication manual of the American psychological association},
  author={American Psychological Association and others},
  year={2010},
  publisher={American Psychological Association}
}

@article{Chen-Zhang-Che-Huang-Han-Yuan-2021, 
    title={Diagnose Like A Pathologist: Weakly-Supervised Pathologist-Tree Network for Slide-Level Immunohistochemical Scoring}, 
    volume={35}, url={https://ojs.aaai.org/index.php/AAAI/article/view/16076}, 
    DOI={10.1609/aaai.v35i1.16076}, 
    number={1}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Chen, Zhen and Zhang, Jun and Che, Shuanlong and Huang, Junzhou and Han, Xiao and Yuan, Yixuan}, 
    year={2021}, 
    month={May}, 
    pages={47-54} }

@article{agcaoglu2020dynamic,
  title={Dynamic resting-state connectivity differences in eyes open versus eyes closed conditions},
  author={Agcaoglu, Oktay and Wilson, Tony W and Wang, Yu-Ping and Stephen, Julia M and Calhoun, Vince D},
  journal={Brain connectivity},
  volume={10},
  number={9},
  pages={504--519},
  year={2020},
  publisher={Mary Ann Liebert, Inc., publishers 140 Huguenot Street, 3rd Floor New~…}
}

@book{inkster2018china,
  title={China’s cyber power},
  author={Inkster, Nigel},
  year={2018},
  publisher={Routledge}
}

@article{guo2023breast,
  title={Breast cancer heterogeneity and its implication in personalized precision therapy},
  author={Guo, Liantao and Kong, Deguang and Liu, Jianhua and Zhan, Ling and Luo, Lan and Zheng, Weijie and Zheng, Qingyuan and Chen, Chuang and Sun, Shengrong},
  journal={Experimental hematology \& oncology},
  volume={12},
  number={1},
  pages={3},
  year={2023},
  publisher={Springer}
}

@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial intelligence and statistics},
  pages={1273--1282},
  year={2017},
  organization={PMLR}
}

@inproceedings{karimireddy2020scaffold,
  title={Scaffold: Stochastic controlled averaging for federated learning},
  author={Karimireddy, Sai Praneeth and Kale, Satyen and Mohri, Mehryar and Reddi, Sashank and Stich, Sebastian and Suresh, Ananda Theertha},
  booktitle={International conference on machine learning},
  pages={5132--5143},
  year={2020},
  organization={PMLR}
}

@article{li2020federated,
  title={Federated optimization in heterogeneous networks},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
  journal={Proceedings of Machine learning and systems},
  volume={2},
  pages={429--450},
  year={2020}
}

@article{acar2021federated,
  title={Federated learning based on dynamic regularization},
  author={Acar, Durmus Alp Emre and Zhao, Yue and Navarro, Ramon Matas and Mattina, Matthew and Whatmough, Paul N and Saligrama, Venkatesh},
  journal={arXiv preprint arXiv:2111.04263},
  year={2021}
}

@inproceedings{li2021model,
  title={Model-contrastive federated learning},
  author={Li, Qinbin and He, Bingsheng and Song, Dawn},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={10713--10722},
  year={2021}
}

@inproceedings{zhang2022federated,
  title={Federated learning with label distribution skew via logits calibration},
  author={Zhang, Jie and Li, Zhiqi and Li, Bo and Xu, Jianghe and Wu, Shuang and Ding, Shouhong and Wu, Chao},
  booktitle={International Conference on Machine Learning},
  pages={26311--26329},
  year={2022},
  organization={PMLR}
}

@inproceedings{zhu2021data,
  title={Data-free knowledge distillation for heterogeneous federated learning},
  author={Zhu, Zhuangdi and Hong, Junyuan and Zhou, Jiayu},
  booktitle={International conference on machine learning},
  pages={12878--12889},
  year={2021},
  organization={PMLR}
}

@article{t2020personalized,
  title={Personalized federated learning with moreau envelopes},
  author={T Dinh, Canh and Tran, Nguyen and Nguyen, Josh},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21394--21405},
  year={2020}
}



@inproceedings{li2021ditto,
  title={Ditto: Fair and robust federated learning through personalization},
  author={Li, Tian and Hu, Shengyuan and Beirami, Ahmad and Smith, Virginia},
  booktitle={International conference on machine learning},
  pages={6357--6368},
  year={2021},
  organization={PMLR}
}

@inproceedings{huang2021personalized,
  title={Personalized cross-silo federated learning on non-iid data},
  author={Huang, Yutao and Chu, Lingyang and Zhou, Zirui and Wang, Lanjun and Liu, Jiangchuan and Pei, Jian and Zhang, Yong},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={35},
  number={9},
  pages={7865--7873},
  year={2021}
}

@inproceedings{luo2022adapt,
  title={Adapt to adaptation: Learning personalization for cross-silo federated learning},
  author={Luo, Jun and Wu, Shandong},
  booktitle={IJCAI: proceedings of the conference},
  volume={2022},
  pages={2166},
  year={2022},
  organization={NIH Public Access}
}

@inproceedings{yang2024fedas,
  title={FedAS: Bridging Inconsistency in Personalized Federated Learning},
  author={Yang, Xiyuan and Huang, Wenke and Ye, Mang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11986--11995},
  year={2024}
}

@article{arivazhagan2019federated,
  title={Federated learning with personalization layers},
  author={Arivazhagan, Manoj Ghuhan and Aggarwal, Vinay and Singh, Aaditya Kumar and Choudhary, Sunav},
  journal={arXiv preprint arXiv:1912.00818},
  year={2019}
}

@article{mireshghallah2020privacy,
  title = {Privacy in Deep Learning: A Survey},
  author = {Mireshghallah, Farinaz and Taram, Mani and Vepakomma, Praneeth and Singh, Anshuman and Raskar, Ramesh and Esmaeilzadeh, Hadi},
  journal = {arXiv preprint arXiv:2004.12256},
  year = {2020}
}

@article{sexton2020gastric,
  title={Gastric cancer: a comprehensive review of current and future treatment strategies},
  author={Sexton, R. E. and Al Hallak, M. N. and Diab, M. and Azmi, A. S.},
  journal={Cancer and Metastasis Reviews},
  volume={39},
  number={4},
  pages={1179--1203},
  year={2020},
  doi={10.1007/s10555-020-09925-3}
}

@article{pfitzner2021federated,
  title={Federated Learning in a Medical Context: A Systematic Literature Review},
  author={Pfitzner, B. and Steckhan, N. and Arnrich, B.},
  journal={ACM Transactions on Internet Technology},
  volume={21},
  number={2},
  pages={1--31},
  year={2021},
  doi={10.1145/3412357}
}

@article{li2020review,
  title={A review of applications in federated learning},
  author={Li, L. and Fan, Y. and Tse, M. and Lin, K.-Y.},
  journal={Computers \& Industrial Engineering},
  volume={149},
  pages={106854},
  year={2020},
  doi={10.1016/j.cie.2020.106854}
}

@article{althnian2021impact,
  title={Impact of Dataset Size on Classification Performance: An Empirical Evaluation in the Medical Domain},
  author={Althnian, A. and AlSaeed, D. and Al-Baity, H. and Samha, A. and Dris, A. B. and Alzakari, N. and Abou Elwafa, A. and Kurdi, H.},
  journal={Applied Sciences},
  volume={11},
  number={2},
  pages={796},
  year={2021},
  doi={10.3390/app11020796}
}

@article{ma2022nonIID,
  title={A state-of-the-art survey on solving non-IID data in Federated Learning},
  author={Ma, X. and Zhu, J. and Lin, Z. and Chen, S. and Qin, Y.},
  journal={Future Generation Computer Systems},
  volume={135},
  pages={244--258},
  year={2022},
  doi={10.1016/j.future.2022.05.003}
}

@article{liang2020think,
  title={Think Locally, Act Globally: Federated Learning with Local and Global Representations},
  author={Liang, Paul Pu and Liu, T. and Liu, Ziyin and Allen, N. B. and Auerbach, R. P. and Brent, D. and Salakhutdinov, R. and Morency, Louis-Philippe},
  journal={arXiv preprint arXiv:2001.01523},
  year={2020}
}

@article{konevcny2017federated,
  title={Federated Learning: Strategies for Improving Communication Efficiency},
  author={Konečný, J. and McMahan, H. B. and Yu, F. X. and Richtárik, P. and Suresh, A. T. and Bacon, D.},
  journal={arXiv preprint arXiv:1610.05492},
  year={2017}
}

@article{sun2023decentralized,
  title={Decentralized Federated Averaging},
  author={Sun, T. and Li, D. and Wang, B.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={4},
  pages={4289--4301},
  year={2023},
  doi={10.1109/TPAMI.2022.3196503}
}

@article{husnoo2023fedrep,
  title={FedREP: Towards Horizontal Federated Load Forecasting for Retail Energy Providers},
  author={Husnoo, Muhammad Akbar and Anwar, A. and Hosseinzadeh, N. and Islam, Shama Naz and Mahmood, Abdun Naser and Doss, R.},
  journal={arXiv preprint arXiv:2203.00219},
  year={2023},
  doi={10.48550/arxiv.2203.00219}
}

@inproceedings{xiaolisha2017scene,
  title={Scene classification with improved AlexNet model},
  author={Xiao, Lisha and Yan, Qin and Deng, Shuyu},
  booktitle={2017 12th International Conference on Intelligent Systems and Knowledge Engineering (ISKE)},
  pages={1--6},
  year={2017},
  doi={10.1109/ISKE.2017.8258820}
}

@inproceedings{he2016deep,
  title={Deep Residual Learning for Image Recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={770--778},
  year={2016},
  doi={10.1109/CVPR.2016.90}
}

@article{howard2017mobilenets,
  title={MobileNets: Efficient Convolutional Neural Networks for Mobile Vision Applications},
  author={Howard, A. G. and Zhu, M. and Chen, B. and Kalenichenko, D. and Wang, W. and Weyand, T. and Andreetto, M. and Hartwig, A.},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}

@article{tan2020efficientnet,
  title={EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
  author={Tan, M. and Le, Q. V.},
  journal={arXiv preprint arXiv:1905.11946},
  year={2020}
}

@article{hu2022gashissdb,
  title={GasHisSDB: A new gastric histopathology image dataset for computer aided diagnosis of gastric cancer},
  author={Hu, Wei and Li, Cheng and Li, Xiaowei and Md Mamunur Rahaman and Ma, Jianrong and Zhang, Yibin and Chen, Hao and Liu, Wei and Sun, Cheng and Yao, Yu-Dong and Sun, Hong and Grzegorzek, Marcin},
  journal={Computers in Biology and Medicine},
  volume={142},
  pages={105207},
  year={2022},
  publisher={Elsevier}
}

@misc{seed2020challenge,
  title={SEED: The challenge of intelligent diagnosis of cancer risk},
  author={{2020 SEED}},
  year={2020},
  howpublished={\url{https://www.jseedata.com/}},
  note={[EB/OL]},
}


@misc{pathological2017challenge,
  title={Pathological Section Identification of AI Challenge},
  year={2017},
  howpublished={\url{http://www.datadreams.org/race-data-3.html}},
  note={[EB/OL]},
}



@misc{fashion-mnist,
  title={fashion\_mnist | TensorFlow Datasets},
  author={{TensorFlow}},
  howpublished={\url{https://www.tensorflow.org/datasets/catalog/fashion_mnist}},
  note={(n.d.)},
}

@misc{cifar10,
  title={cifar10 | TensorFlow Datasets},
  author={{TensorFlow}},
  howpublished={\url{https://www.tensorflow.org/datasets/catalog/cifar10}},
  note={(n.d.)},
}

@article{yosinski2015understanding,
  title={Understanding Neural Networks Through Deep Visualization},
  author={Yosinski, Jason and Clune, Jeff and Nguyen, Anh Mai and Fuchs, Thomas J. and Lipson, Hod},
  journal={ArXiv (Cornell University)},
  year={2015},
  doi={10.48550/arxiv.1506.06579}
}



@misc{adaloglou2020receptive,
  title={Understanding the receptive field of deep convolutional networks},
  author={Adaloglou, Nikos},
  howpublished={\url{https://theaisummer.com/receptive-field/}},
  note={AI Summer, 2020, July 2},
}

@article{dinh2020personalized,
  title={Personalized Federated Learning with Moreau Envelopes},
  author={Dinh, Canh T. and Tran, Nguyen H. and Nguyen, Jianyu},
  journal={Neural Information Processing Systems},
  volume={33},
  pages={21394--21405},
  year={2020}
}

@inproceedings{tan2022fedproto,
  title={FedProto: Federated Prototype Learning across Heterogeneous Clients},
  author={Tan, Yongxin and Long, Guodong and Liu, Lina and Zhou, Tianyi and Lu, Qiang and Jiang, Jing and Zhang, Chengqi},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={36},
  number={8},
  pages={8432--8440},
  year={2022},
  doi={10.1609/aaai.v36i8.20819}
}

@article{tan2022contrastive,
  title={Federated Learning from Pre-Trained Models: A Contrastive Learning Approach},
  author={Tan, Yongxin and Long, Guodong and Ma, Jian and Liu, Lina and Zhou, Tianyi and Jiang, Jing},
  journal={ArXiv (Cornell University)},
  year={2022},
  doi={10.48550/arxiv.2209.10083}
}

@article{xu2023personalized,
  title={Personalized Federated Learning with Feature Alignment and Classifier Collaboration},
  author={Xu, Jing and Tong, Xin and Huang, Shu-Lei},
  journal={ArXiv (Cornell University)},
  year={2023},
  doi={10.48550/arxiv.2306.11867}
}




==> related_old.tex <==


 SCAFFOLD, FedProx, and FedDyn are improvements to FedAvg that address heterogeneity challenges in federated learning. SCAFFOLD \cite{karimireddy2020scaffold} introduces a variance reduction mechanism to handle non-IID client data by implementing a distributed optimization step to limit model bias. FedProx \cite{li2020federated} adds a proximity term to reduce the difference between local and global objectives, allowing devices to complete varying amounts of computation based on their resources. FedDyn \cite{acar2021federated} employs a dynamic regulariser to simultaneously minimize local and global experience loss, updating each device's local risk objective based on the global optimum in each training round.

The goal of traditional FL is to train a generic global model that performs well for all clients. Traditional FL is easy to deploy and suitable for small sample scenarios with consistent data distribution. However, it performs poorly when dealing with heterogeneous data and cannot generate personalised models for customers when dealing with non-iid data. To address this problem, personalized federated learning (pFL) has introduced various techniques to balance global optimization and personalization needs. The goal of personalized FL is to train a local model for each client that is more suitable for local data. They enable customers not only to contribute to training global models but also to adapt personalised models to local data characteristics. Their main advantage is that they can strike a balance between personalisation and global collaboration, thereby achieving strong model performance in heterogeneous data environments. However, as the number of customers increases, these models face increased communication costs and computational complexity, which may affect overall efficiency.

Regularisation-based personalized federated learning methods (pFL) were developed to solve the problem of non-IID data. In particular, pFedMe introduces the Moreau envelope into the client loss function, which transforms the personalized federated learning problem into a two-layer optimization problem, thereby optimizing both the global model and the personalized model. The introduction of the Moreau envelope smooths the original objective function, simplifies the optimization process, and speeds up convergence. Studies have shown that pFedMe exhibits faster convergence and better model performance when dealing with non-IID data sets \cite{t2020personalized}.  Ditto, another regularisation-based personalised federated learning method, adds a regularisation term to the multi-task learning framework to achieve a balance between personalisation and global objectives \cite{li2021ditto}. Ditto allows each client to learn a personalised model while leveraging information from the global model to improve the overall result. By adjusting the hyperparameter, Ditto can flexibly control the degree of personalisation: when the hyperparameter is set to the minimum value, it is equivalent to training only a local personalised model; when the hyperparameter is increased, the model gradually converges towards the global objective. 

 The advantage of adding a regularisation term, the objectives of the global model and the local personalised model can be balanced, personalised learning can be achieved, and the convergence speed can be accelerated to a certain extent. However, model tuning becomes more difficult. Higher computational complexity also places higher hardware requirements. When data heterogeneity is very serious, the regularisation term may not be sufficient to fully solve the problem.

 Personalized-aggregation-based pFL is an advanced method in the field of federated learning that focuses on enhancing personalization at the aggregation stage. It allows the server to dynamically adjust the aggregation weights based on the unique parameters of each client, making the global model more adaptable to the needs of individual clients. FedAMP introduces the attention message passing (AMP) mechanism\cite{huang2021personalized}. This feature is designed to facilitate collaborative learning by adaptively adjusting the sharing of model parameters between clients. The similarity of model parameters between clients is used as the weight for updating, facilitating collaboration between clients with similar data distributions. This approach enables the federated system to adaptively modify shared parameters, enhancing personalisation through continuous fine-tuning. Similarity then adjusts the regularisation strength accordingly, ensuring that each client receives more relevant updates based on their unique data characteristics. However, FedAMP can affect the personalised performance of the model by inadvertently reducing personalisation when the regularisation parameter is too large, ignoring local client objectives.  FedApple and FedAS frameworks are another two key models in Personalized-aggregation-based pFL. FedApple \cite{luo2022adapt} tackles cross-domain adaptation through a core model and directed relationships (DRs), reducing communication costs via selective parameter sharing while preserving privacy, though it increases computational complexity through its iterative process. FedAS \cite{yang2024fedas} addresses data heterogeneity and client inconsistency using parameter alignment and client synchronization mechanisms, where the Fisher information matrix guides contribution weight adjustments, but its requirement for consistent model architectures limits its applicability in diverse client environments. 

 The advantage of personalized-aggregation-based pFL models is that they enhance collaboration between clients through dynamic adjustment mechanisms, improving personalization, particularly in environments with high data heterogeneity. However, the high computational costs may weaken the retention of personalized features, especially when computational resources are limited.

  Model-splitting-based personalized FL that divides the model into shared and personalized layers was first proposed in the paper which introduce the FedPer. \cite{arivazhagan2019federated}. The shared layers transmit global information between clients, while the personalized layers are trained independently on local data. This approach ensures global collaboration while preserving personalized characteristics. However, fixed layer selection might not fully capture the most representative feature layers of each client.

 The advantage of model-splitting-based pFL models is their ability to balance global collaboration and personalized characteristics, making them suitable for heterogeneous data environments. At the same time, fewer model parameters are uploaded, which reduces communication costs. However, the fixed layer selection may limit personalization, as it lacks the flexibility to address the varying feature needs of different clients.

 The proposal of federated learning can greatly support cancer image recognition tasks and effectively alleviate the problem of insufficient samples caused by the imbalance of medical institution resources while protecting data privacy. Traditional federated learning methods excel at constructing stable global models but have obvious limitations when dealing with heterogeneous data. In recent years, personalized federated learning has introduced various innovative techniques. Personalized federated learning methods balance personalization and global collaboration, significantly improving model performance under non-IID data and meeting the personalized needs of customers. However, each type of FL model has its own advantages and disadvantages in terms of communication costs, computational efficiency, and personalisation. Finding the right balance between these is still a core research direction for the future.

 By studying the existing literature, we have gained inspiration for an innovative FL framework. To address heterogeneity, personalised aggregation methods are considered, using an attention message passing mechanism, and the distance between model parameters is used to measure the similarity of local data distributions as a weighted average weight to meet customer personalisation needs. In addition, to ensure that the learned information is valid, the FIM metric is used to measure the global contribution of parameters. Finally, a model splitting mechanism is considered to reduce communication costs. Based on existing research, we propose our own innovative framework, which aims to effectively address these challenges.
  
  
